Cutting a tree with Subgraph Complementation is hard, except for some small trees

For a graph property $\Pi$, Subgraph Complementation to $\Pi$ is the problem to find whether there is a subset $S$ of vertices of the input graph $G$ such that modifying $G$ by complementing the subgraph induced by $S$ results in a graph satisfying the property $\Pi$. We prove that the problem of Subgraph Complementation to $T$-free graphs is NP-Complete, for $T$ being a tree, except for 41 trees of at most 13 vertices (a graph is $T$-free if it does not contain any induced copies of $T$). This result, along with the 4 known polynomial-time solvable cases (when $T$ is a path on at most 4 vertices), leaves behind 37 open cases. Further, we prove that these hard problems do not admit any subexponential-time algorithms, assuming the Exponential Time Hypothesis. As an additional result, we obtain that Subgraph Complementation to paw-free graphs can be solved in polynomial-time.

==> 5-connected-duplicated.tex <==
\section{5-connected graphs with duplicated vertices}
\label{sec:5-connected-duplicated}

\begin{lemma}
\label{lem:5-conn-dupe}
    Let $H'$ be a connected, non self-complementary, prime graph %with an independent set $I$ of size 4 or 
    with a clique $K$ of size 4. Let $H$ be a 5-connected, non self-complementary graph with the following properties satisfied:
    \begin{enumerate}[label=(\roman*)]
        \item $H'$ is the quotient graph of $H$. 
        \item $H$ has a clique $K_4$  such that the vertices in $K_4$ has no twins. 
    \end{enumerate}
   
\end{lemma}


    Let $H'$ be a connected, non self-complementary, prime graph with %an independent set $I$ of size 4 or     with 
    a clique $K_4$. % of size 4. 
    Let $H$ be a 5-connected, non self-complementary graph such that $H'$ is the quotient graph of $H$. 
    Assume that $H$ satisfies the conditions of Lemma \ref{lem:5-conn-dupe}.
    Let $H$ contains $t$ vertices out of which $p$ vertices do not have any twins in $H$.
    Let $V(H)=\{v_1,v_2,\ldots,v_t\}$.
    Without loss of generality assume that these $p$ vertices, denoted by $\{v_1,v_2,\ldots,v_p\}$ induces a $K_4$ % or $4K_1$ 
    in $H$.
    The remaining $k=t-p$ vertices have twins in $H$.
    Thus, $H'$ has $t'=p+k'$ vertices.
    Let $\mathcal{M}=\{M_1,M_2,\ldots,M_{t'}\}$ be the modular decomposition of $H$, where $t'=k'+p$, where $k'$ is the number of modules containing twins.
    Let $\{M_1,M_2,\ldots, M_p\}$ forms the modules ($M_i= \{v_i\}$, for $1\leq i\leq p$) containing the non-twin vertices, and $\{M_{p+1}, M_{p+2}, \ldots, M_{t'}\}$ forms the modules containing twins.
    Let $r$ be the maximum size of modules containing twins, i.e., $r= max_{i={p+1}}^{i=t'}\{|M_i|\}$.
    Let $H'$ be the quotient graph of $H$. By $R$, we denote the graph $\overline{H}[K_j]$, i.e., $R$ is the graph obtained from $\overline{H}$ by replacing each vertex by a clique of size $r$.
    
    

==> Tree/leaves_duplicated.tex <==
\subsection{One of the leaves of a path is duplicated}
\label{sec:leaves duplicated}

Let $T'$ be a path on $t$ vertices and $T$ be a tree on $t+1$ vertices obtained by duplicating one of the leaves of $T'$.

\begin{construction}
\label{cons tree duplicated}
    Given a graph $G'$, the graph $G$ is constructed from $G'$ as follows: 
    for each vertex $u$ of $G'$ replace $u$ with a set $W_u$ which induces a $2K_2$.
    The so obtained graph is $G$ (see Figure %~\ref{fig cons tree duplicated} 
    for an example). 
\end{construction}

 \begin{figure}[!htbp]
    \begin{subfigure}[b]{0.50\textwidth}
          \centering
          \resizebox{0.8\linewidth}{!}{\input{figs/Tree/G'-leaves duplicated}}  
          \caption{$G'$}
          \label{fig:A}
     \end{subfigure}
     \begin{subfigure}[b]{0.50\textwidth}
          \centering
          \resizebox{0.8\linewidth}{!}{\input{figs/Tree/G-leaves duplicatd}}  
          \caption{$G$}
          \label{fig:B}
     \end{subfigure}
   \label{fig:leaves duplicated}
   
     \caption{{An example of Construction \ref{cons tree duplicated}. In both $G'$ (\ref{fig:A}) and $G$ (\ref{fig:B}), circles represent a vertex. The lines connecting two circles indicate that the vertices corresponding to that circles are adjacent. Similarly, the lines connecting two circles (dashed) indicate that all the vertices in one circle (dashed) is adjacent to all the vertices in other circle (dashed)}}.
     
\end{figure}

This brings us to our first lemma. 

\begin{lemma}\label{lem tree duplicated if}
   If $G' \oplus S' \in \mathcal{F}(T')$ for some $S' \subseteq V(G')$, then   $G \oplus S \in \mathcal{F}(T)$, where $S$ contains each set $W_u$ of vertices in $G$ corresponding to the vertex $u$ in $S'$.
\end{lemma}

\begin{proof}
    Let a $T$ be induced by $A$ (say) in $G\oplus S$. 
   % Now consider a set $B$ in $G'\oplus S'$.
    Recall that $G$ is constructed by replacing each vertex $u$ in $G'$ with a module $W_u$ which induces a $2K_2$.
    Now consider the $2K_1$ in $T$ of $G\oplus S$ which induces a module.
    %  Thus, for the $2K_1$ in $T$ of $G\oplus S$ which induces a module there will be at least one vertex $u\in G'\oplus S'$.
    Suppose the vertices in this $2K_1$ are from a module $W_u\in G\oplus S$, then there exist a vertex $u$ in $G'\oplus S'$ such that $u$ in $G'$ is replaced with $W_u$ in $G$--note that even if a module $W_u$ which induces a $2K_2$ is in $S$ or a part of it is in $S$, $G\oplus S$ contains a $2K_1$.
    Now, if the vertices in this $2K_1$ are obtained from two different modules $W_u$ and $W_v$, then it means that the false twin vertices $u$ and $v$ in $G'$ are replaced with $W_u$ and $W_v$  in $G$.
    Thus, for each vertex or a $2K_1$ which induces a module in $A$, there will be at least one vertex $u\in G'\oplus S'$ corresponding to that vertex or $2K_1$ in $G\oplus S$. 
    Assume that the set $B$ of vertices in $G'\oplus S'$ is obtained by including the vertices which are corresponding to the vertices or modules in $T$ of $G\oplus S$.
   % If a vertex or a module which induces a $2K_1$ in $G\oplus S$ is in $A$, then corresponding vertices in $G'\oplus S'$ is placed in $B$.
    This implies that the set $B$  induces a $T'$ in $G'\oplus S'$ as the way it is constructed. 
    However, that is not possible according to the statement of the lemma. 
\end{proof}

The converse of the lemma turns out to be true as well. 

\begin{lemma}\label{lem tree ind onlyif}
   If $G \oplus S \in \mathcal{F}(T)$ for some $S \subseteq V(G)$, then   $G' \oplus S' \in \mathcal{F}(T')$, where $S'$ is the set of vertices obtained in such a way that whenever a $K_2$ from a module $W_u$ (which induces a $2K_2$) is in $S$, the corresponding vertex $u$ in $G'$ is included in $S'$.
\end{lemma}

\begin{proof}
  Suppose $G' \oplus S'$ contains a $T'$ induced by $A$ (say). 
  Since $G$ is constructed from $G'$ by replacing each vertex $u$ in $G'$ with a module $W_u$ which induces a $2K_2$. 
  Thus, for each vertex $u$ in $T'$ in $G'\oplus S'$, there will be a set $W_u$ in $G \oplus S$.
  We know that a vertex $u\in G'$ is not in the solution $S'$ implies that at least one vertex from each copy of the $K_2$ in $2K_2\in W_u$ is not in the solution $S$. Thus, the vertices in $W_u\setminus S$ together induces a $2K_1$ in $W_u$.
  This means that, even if the set $W_u$ is in $S$ or a part of it is in $S$, a $2K_1$ is induced by the vertices in $W_u$.  Thus, there will be a $T$ in $G$. 
  Therefore, we can conclude that there is no induced $T'$ in $G' \oplus S'$. 
  
\end{proof}





==> figs/5-connected/K4complement.tex <==
\begin{tikzpicture}  [myv/.style={circle, draw, inner sep=2pt},myv1/.style={rectangle, draw},myv2/.style={rectangle, draw,dotted},myv3/.style={circle, draw, inner sep=0.5pt},my/.style={\input{figs/hard/c},draw}, myv4/.style={rectangle, draw,dashed,color=red}] 
 
% following are the six nodes in  $V_i$
\node[myv] (x1) at (-1,4.5) {};
\node[myv] (x2) at (0.3,4.5) {};
\node[myv] (x3) at (1.7,4.5) {};
\node[myv] (x4) at (3,4.5) {};
\node[myv] (a1) at (-1,3.5) {};
\node[myv] (a2) at (0,3.5) {};
\node[myv] (a3) at (1,3.5) {};
\node[myv] (a4) at (2,3.5) {};
\node[myv] (a5) at (3,3.5) {};
%\node[myv] (a6) at (6.5,5) {$v_4$};
\node[myv] (a7) at (1,5.5)  {};


 
 
 \draw  (x1) -- (a7);   
 \draw  (x2) -- (a7);
 \draw  (x3) -- (a7);
 \draw  (x4) -- (a7);
 \draw  (a1) -- (x1);
 \draw  (a1) -- (x2);
 \draw  (a2) -- (x2);
 \draw  (a3) -- (x2);
 \draw  (a3) -- (x3);
 \draw  (a4) -- (x3);
 \draw  (a4) -- (x4);
 \draw  (a5) -- (x4);
 \draw  (a1) -- (a2);
 \draw  (a3) -- (a2);
 \draw  (a1) to[bend right=25] (a4);
 \draw  (a2) to[bend right=25] (a5);
 \draw  (a3) to[bend right=35] (a5);
 \draw  (a4) -- (a5);
 
 

% \draw  (a6) -- (x);
 
 
  
 % \draw (x1) -- (x2);
  %\draw (x1) to[bend right=15] (x3);
  %\draw (x1) to[bend right=20] (x4);
  %\draw (x2) -- (x3);
  %\draw (x2) to[bend right=15] (x4);
  %\draw (x3) -- (x4);
  

  
 
  
 
  
\end{tikzpicture}  


==> figs/open/C112.tex <==
\fbox{\begin{tikzpicture}[myv/.style={circle, draw, inner sep=1.5pt}]
  \node (z) at (0,0) {};

  \node[myv] (a) at (0,0.6) {};
  \node[myv] (b) at (0,0.3) {};
  \node[myv] (c) at (-0.3,0.3) {};
  \node[myv] (d) at (0.3,0.3) {};
  \node[myv] (e) at (0.3,0) {};

  \draw (a) -- (b);
  \draw (a) -- (c);
  \draw (a) -- (d);
  \draw (d) -- (e);

\end{tikzpicture}}


==> non-prime.tex <==
\section{Non-prime graphs}
\label{H-free prime to non- prime}

\input{5-connected/quotient}
\sandeep{Please go through: \cite{DBLP:journals/csr/HabibP10}. We need to clearly understand and write what we mean by a modular partition. Please use the 
definitions in the cited paper. We are actually talking about maximal strong modules. We have to take the assumption that neither $H$ nor $\overline{H}$
is connected. Then we can use the Theorem 2 of the paper. Refer to Gallai's original paper as well.} 
Let $H$ be a non-prime graph and $H'$ be the quotient graph of $H$. Let $M_1,M_2,\ldots, M_l$ be the distinct strong modules in $H$. 
%\sandeep{Use capital letters for modules. Define box product in preliminaries.}
Now consider a set $M$ of vertices which induces a $(M_1\square M_2 \square \ldots \square M_l)\square(\overline{M_1\square M_2 \square \ldots \square M_l})$. %(which is also a tree).Let $j$ be the maximum number of leaves for a vertex in $T$.% module of the quotient graph of $T$

\begin{construction}
\label{cons gen ind}
     Given a graph $G'$, the graph $G$ is constructed from $G'$ as follows: 
     for each vertex $u$ of $G'$ replace $u$ with a set $W_u$ which induces a $(M_1\square M_2 \square \ldots \square M_l)\square(\overline{M_1\square M_2 \square \ldots \square M_l})$. % where $j$ is the maximum number of vertices in a module of the quotient graph of $T$. %for a vertex in $T$. 
    The so obtained graph is $G$ (see Figure %~\ref{pt cons} 
    for an example). 
\end{construction}
%\sandeep{Define what it means by replacing a vertex with a graph in preliminaries.}
This brings us to our first lemma. 

\begin{lemma}\label{lem gen ind if}
   If $G' \oplus S' \in \mathcal{F}(H')$ for some $S' \subseteq V(G')$, then   $G \oplus S \in \mathcal{F}(H)$, where $S$ contains set $W_u$ of vertices in $G$ corresponding to each vertex $u$ in $S'$.
\end{lemma}

\begin{proof}
    By Lemma \ref{quotient}, it is clear that, $H$ is not induced by a module $W_u$ in $G$.
    Recall that $G$ is obtained by replacing each vertex $u$ in $G'$ by a set $W_u$ which induces a $(M_1\square M_2 \square \ldots \square M_l)\square(\overline{M_1\square M_2 \square \ldots \square M_l})$.
    Suppose the vertices in $M_i$ of $H$ are from a module $W_u\in G$, then there exist a vertex $u$ in $G'$ such that $u$ is replaced with $W_u$ in $G$. 
    If the $M_i$ is induced by the vertices from two different modules $W_u$ and $W_v$, then it means that $W_u$ and $W_v$ in $G$ are replaced with the twin (either true twin or false twin) vertices $u$ and $v$   in $G'$.
    Thus, if $H$ is induced by $A$(say) in $G$, then for each module $M_i$ in the $H$, there will be at least one vertex $u$ in $G'$ corresponding to the module $M_i$. %\sandeep{I do not understand this}
    The so obtained graph $B$ in $G'$ induces an $H'$ as $B$ is obtained with the vertices in $G'$ corresponding to the each $M_i$s in $H$ of $G$. % by a single vertex in $G'$.
    However, that is not possible according to the statement of the lemma. 
\end{proof}

The converse of the lemma turns out to be true as well. 

\begin{lemma}\label{lem gen ind onlyif}
   If $G \oplus S \in \mathcal{F}(H)$ for some $S \subseteq V(G)$, then   $G' \oplus S' \in \mathcal{F}(H')$, where $S'$ is the set of vertices obtained in such a way that whenever a $\overline{M_1\square M_2\square\ldots \square M_l}$ from a module $W_u$ (which induces a $(M_1\square M_2 \square \ldots \square M_n)\square(\overline{M_1\square M_2 \square \ldots \square M_n})$) is in $S$, the corresponding vertex $u$ in $G'$ is included in $S'$.
\end{lemma}


\begin{proof}
  Suppose $G' \oplus S'$ contains an $H'$ induced by $A$ (say). 
  Since $G$ is constructed from $G'$ by replacing each vertex $u$ in $G'$ with a module $W_u$, for each vertex $u$ in $A$, there will be a set $W_u$ in $G \oplus S$. We know that a vertex $u\in G'$ is not in the solution $S'$ implies that at least one vertex from each copy of $\overline{M_1\square M_2 \square \ldots \square M_n}$ of $W_u$ is not in the solution. Thus, the vertices in $W_u\setminus S$ together induces a $M_1\square M_2 \square \ldots \square M_n$ in $W_u$. This means that, even if the set $W_u$ is in $S$ or a part of it is in $S$, an $M_1\square M_2 \square \ldots \square M_n$ is induced by the vertices in $W_u$.  Thus, there will be an $H$ in $G$. Therefore, we can conclude that there is no induced $H'$ in $G' \oplus S'$. 
  
\end{proof}
